Inverse Scale Space Iterations for Non-Convex Variational Problems: The Continuous and Discrete Case

Non-linear filtering approaches allow to obtain decompositions of images with respect to a non-classical notion of scale, induced by the choice of a convex, absolutely one-homogeneous regularizer. The associated inverse scale space flow can be obtained using the classical Bregman iteration with quadratic data term. We apply the Bregman iteration to lifted, i.e. higher-dimensional and convex, functionals in order to extend the scope of these approaches to functionals with arbitrary data term. We provide conditions for the subgradients of the regularizer -- in the continuous and discrete setting -- under which this lifted iteration reduces to the standard Bregman iteration. We show experimental results for the convex and non-convex case.

==> Sections/ContLiftedBreg.tex <==
\section*{Continuous Formulation of Lifted Bregman}

\subsection*{Calibration based lifting}

We consider variational image processing problems with energies of the form
\bfln
F(u) := \into \rho(x,u(x)) \dx + \into \eta(\nabla u(x)) \dx.
\label{eq:problem}
\efln
The lifted convex version $\mathcal{F}$  of the functional $F$ is defined as:
\bfl
\mathcal{F}(v) := \sup_{\phi \in \mathcal{K}} \intog \langle \phi, Dv \rangle ,
\label{eq:lifted_F}
\efl
where $v:\Omega\times\R\mapsto [0,1 ]$ with distributional derivative $Dv$ and the admissible dual vector fields are given by
\bfln
\mathcal{K} := \{ (\phi_x, \phi_t) \in & C_0(\Omega\times\R; \R^d\times\R ):  \\ & \phi_t(x,t) + \rho(x,t) \geq \eta^*(\phi_x(x,t)), \\
&  \forall (x,t) \in \Omega\times\R \} .
\label{eq:constraint_set_K}
\efln
%
In case of the TV regularizer, which is a convex one-homogeneous function, the conjugate can be written as the indicator function of a convex set. Thus, the constraint set $\mathcal{K}$ can be separated as follows:
\begin{align}
\label{eq:constraint_set_Kt}
\mathcal{K}_t := \{ \phi_t \in & C_0(\Omega\times\R; \R ):  \quad - \phi_t(x,t) \leq  \rho(x,t), \quad  \forall (x,t) \in \Omega\times\R \} , \\  
\mathcal{K}_x := \{ \phi_x \in & C_0(\Omega\times\R; \R^d):  \quad  \phi_x(x,t) \in \text{dom} \{ \eta^*\} , \quad  \forall (x,t) \in \Omega\times\R \} ,
\label{eq:constraint_set_Kx}
\end{align}
and \eqref{eq:lifted_F} is equal to
\bfl
\mathcal{F}(v) := \sup_{\substack{\phi_x \in \mathcal{K}_x \\ \phi_t \in \mathcal{K}_t} } \intog \left \langle \begin{pmatrix} \phi_x \\ \phi_t \end{pmatrix}, Dv \right \rangle ,
\label{eq:lifted_F_Ksep}
\efl


 
\subsection*{Bregman}

In each Bregman iteration we solve the minimization problem 
\bfl
u_k & \in \arg\min_{u} F(u) - \emphr{\langle p_{k-1}, u \rangle} .
\label{eq:breg_uk}
\efl
where $p_{k-1} \in \partial\into \eta(\nabla u_{k-1}(x)) \dx$. Since the linear term in \eqref{eq:breg_uk} does not depend on $\nabla u$ and we can reinterpret the problem by extending our original data term:
\begin{align}
\label{eq:problem_xi}
F_\xi(u) & := \into \xi(x,u(x)) \dx + \into \eta(\nabla u(x)) \dx ,\\ 
\xi(x,u(x)) & :=  \rho(x,u(x)) - p_{k-1}(x)u(x) ,
\end{align}
thus solving 
\bfl
u_k & \in \arg\min_{u} F_\xi(u)
\label{eq:breg_uk_xi}
\efl
in each Bregman iteration. Using the theory of calibration based lifting we rewrite \eqref{eq:breg_uk_xi} as
\begin{align}
\mathcal{F}(v) &:= \sup_{\substack{\phi_x \in \mathcal{K}_x \\ \phi_t \in \mathcal{K}_t} } \intog \left \langle \begin{pmatrix} \phi_x \\ \phi_t \end{pmatrix}, Dv \right \rangle , \\
\mathcal{K}_{t,\xi} &:= \{ \phi_t \in  C_0(\Omega\times\R; \R ):  \quad - \left( \phi_t(x,t) - t p_{k-1}(x) \right)  \leq  \rho(x,t), \quad  \forall (x,t) \in \Omega\times\R \} , \\  
\mathcal{K}_x &:= \{ \phi_x \in  C_0(\Omega\times\R; \R^d):  \quad  \phi_x(x,t) \in \text{dom} \{ \eta^*\} , \quad  \forall (x,t) \in \Omega\times\R \} ,
\end{align}

Now we substitute  $\phi_t^p(x,t) :=   \phi_t(x,t) - t p_{k-1}(x)$ \db{$\in C_0 (\otg; \R)?!$} which leads to 
\begin{align}
\mathcal{F}(v) &:=  \sup_{\substack{\phi_x \in \mathcal{K}_x \\ \phi_t^p \in \mathcal{K}_t} } \intog \left \langle \begin{pmatrix} \phi_x \\ \phi_t^p(x,t) + t p_{k-1}(x) \end{pmatrix}, Dv \right \rangle , \\
&= \sup_{\substack{\phi_x \in \mathcal{K}_x \\ \phi_t^p \in \mathcal{K}_t} } \intog \left \langle \begin{pmatrix} \phi_x \\ \phi_t^p \end{pmatrix}, Dv \right \rangle + \emphr{\intog \langle t p_{k-1}(x), (Dv)_t \rangle}, \label{eq:lifted_linear_term}\\
%
\mathcal{K}_t &:= \{ \phi_t^p \in  C_0(\Omega\times\R; \R ):  \quad - \phi_t^p(x,t)  \leq  \rho(x,t), \quad  \forall (x,t) \in \Omega\times\R \} , \\ 
%
\mathcal{K}_x &:= \{ \phi_x \in  C_0(\Omega\times\R; \R^d):  \quad  \phi_x(x,t) \in \text{dom} \{ \eta^*\} , \quad  \forall (x,t) \in \Omega\times\R \} ,
\end{align}

\subsubsection*{Equivalence}

For any $u:\Omega\to\Gamma$ with graph $v:\otg\to[0,1]$:
\beq
v(x,t) = \begin{cases}
1, & u(x) \geq t ,  \\
0, & u(x) < t , 
\end{cases}
\eeq
the distributional derivative of $v$ w.r.t.~ t is given by 
\beq
(Dv)_t = \begin{cases}
-1, & u(x) = t , \\
0, & \text{else}.
\end{cases}
\eeq 
\emphr{An immediate consequence for \eqref{eq:lifted_linear_term} is
\bfl
\intog \langle t p_{k-1}(x), (Dv)_t \rangle &=  - \into p_{k-1}(x) u(x) \dx  \\ &= - \into p_{k-1}(x) \int_\Gamma v(x,t) \dt \dx \\ &= - \intog p_{k-1}(x) v(x,t) \dxt .
\efl }

\subsubsection*{QUESTION}

Connection between $\partial TV(G_u)$ and $\partial TV(u)$?

\begin{enumerate}
\item[$\partial TV(u):$] For fixed $u\in\BV(\Omega;\Gamma)$ we have  $p\in\partial\TV(u)$ iff
\[  
TV(v) \geq TV(u) + \langle p, v- u \rangle, \quad \forall v\in\BV(\Omega;  \Gamma).
\]
\item [$\partial TV(G_u):$] Let $G_u:\Omega\times\Gamma\to\{0,1\}$ denote the full graph of $u$ and let $\bs{v}:\Omega\times\Gamma\to[0,1]$ be arbitrary. We make the following observations:
\begin{enumerate}
\item It holds:
\[ TV(G_u) = TV(u).\]
\item It does not hold:
\[ TV(\bs{v}) = TV(\mathbbm{1}_{v\geq s}) \quad \text{for  a.e. } s \in (0,1). \]
\end{enumerate}
Now we show, that $\bs{p}:\otg\to\R, \, \bs{p}(x,t)\mapsto p(x)$ is a subgradient of $TV(G_u)$, i.e.
\bfl
TV(\bs{v}) & \geq TV(G_u) + \langle \bs{p}, \bs{v}- G_u \rangle, \quad \forall \bs{v}\in\BV(\otg ; [0,1]) \\
\Leftrightarrow TV(\bs{v}) & \geq TV(u) + \langle \bs{p}, \bs{v} \rangle - \langle \bs{p},  G_u \rangle, \quad \forall \bs{v}\in\BV(\otg ;  [0,1])  \\
\Leftrightarrow TV(\bs{v}) & \geq TV(u) + \langle \bs{p}, \bs{v} \rangle - \langle p,  u \rangle, \quad \forall \bs{v}\in\BV(\otg ;  [0,1]) \\
\Leftrightarrow TV(\bs{v}) -  \langle \bs{p}, \bs{v} \rangle & \geq TV(u)  - \langle p,  u \rangle, \quad \forall \bs{v}\in\BV(\otg ;  [0,1]).
\efl
We know:
\bfl
TV(v) - \langle p, v \rangle \geq TV(u) - \langle p, u \rangle, \quad \forall v\in\BV(\Omega; \Gamma).
\efl
Last equivalence can easily be shown:
\bfl
\langle \bs{p},  G_u \rangle &= \intog \bs{p}(x,t) G_u(x,t) \dxt \\
&= \into p(x) \int_0^{u(x)} 1 \dt \dx \\
&= \into p(x)u(x) \dx \\
&= \langle p,  u \rangle
\efl
Now it would be tremendous if we could show
$TV(\mathbbm{1})$
\end{enumerate}


==> Sections/calibration_bregman.tex <==
\section{Calibration Bregman}

We consider variational image processing problems with energies of the form
\bfln
F(u) := \into \rho(x,u(x)) \dx + \into \eta(\nabla u(x)) \dx.
\label{eq:problem}
\efln
[...] The lifted convex version $\mathcal{F}$  of the functional $F$ is defined as:
\bfln
\mathcal{F}(v) := \sup_{\phi \in \mathcal{K}} \int_{\Omega \times \Gamma} \langle \phi, Dv \rangle ,
\label{eq:lifted_F}
\efln
where $v:\Omega\times\R\mapsto [0,1 ]$ with distributional derivative $Dv$ and the admissible dual vector fields are given by
\bfln
\mathcal{K} := \{ (\phi_x, \phi_t) \in & C_0(\Omega\times\R; \R^d\times\R ):  \\ & \phi_t(x,t) + \rho(x,t) \geq \eta^*(\phi_x(x,t)), \\
&  \forall (x,t) \in \Omega\times\R \} .
\label{eq:constraint_set_K}
\efln
%
Now let us recall the definition of the Bregman iteration: \\

 \noindent              \fbox{%
                \begin{minipage}[t]{0.95\linewidth}
                \textbf{Algorithm 1: Bregman iteration}
                        \begin{itemize}
                        \item[] Initialize $p_0 = 0$ and repeat for $k = 1,2,...$
                                                \begin{flalign}
                                u_k & \in \arg\min_{u} F(u) - \langle p_{k-1}, u \rangle , \label{eq:breg_uk}\\
                                %q_{k} & \in - \partial H(u_k) + q_{k-1} \label{eq:breg_qk}. 
                                p_{k} & \in \partial\into \eta(\nabla u_k(x)) \dx \label{eq:breg_qk}. 
                        \end{flalign}                   
                        \end{itemize}                                           
                \end{minipage}} \\
The linear term in \eqref{eq:breg_uk} does not depend on $\nabla u$ and we can reinterpret the problem by extending our original data term:
\bfln
F_\xi(u) & := \into \xi(x,u(x)) \dx + \into \eta(\nabla u(x)) \dx \\ 
\xi(x,u(x)) & :=  \rho(x,u(x)) - p_{k-1}(x)u(x) .
\label{eq:problem}
\efln
Then the Bregman iteration can be rewritten as:  \\

 \noindent              \fbox{%
                \begin{minipage}[t]{0.95\linewidth}
                \textbf{Algorithm 1: Bregman iteration}
                        \begin{itemize}
                        \item[] Initialize $p_0 = 0$ and repeat for $k = 1,2,...$
                                                \begin{flalign}
                                u_k & \in \arg\min_{u} F_\xi(u) , \label{eq:breg_uk_2}\\
                                %q_{k} & \in - \partial H(u_k) + q_{k-1} \label{eq:breg_qk}. 
                                p_{k} & \in \partial\into \eta(\nabla u_k(x)) \dx \label{eq:breg_qk}. 
                        \end{flalign}                   
                        \end{itemize}                                           
                \end{minipage}} \\ 
Now we can rewrite line \eqref{eq:breg_uk_2} as a lifted problem
\bfln
\mathcal{F}_\xi(v) := \sup_{\phi \in \mathcal{K}_\xi} \int_{\Omega \times \Gamma} \langle \phi, Dv \rangle ,
\label{eq:lifted_F_xi}
\efln
where $v:\Omega\times\R\mapsto [0,1 ]$ with distributional derivative $Dv$ and the admissible dual vector fields are given by
\bfln
\mathcal{K}_\xi := \{ (\phi_x, \phi_t) \in & C_0(\Omega\times\R; \R^d\times\R ):  \\ & \phi_t(x,t) + \xi(x,t) \geq \eta^*(\phi_x(x,t)), \\
&  \forall (x,t) \in \Omega\times\R \} .
\label{eq:constraint_set_K_xi}
\efln

This results in the following lifted Bregman iteration: \\

 \noindent              \fbox{%
                \begin{minipage}[t]{0.95\linewidth}
                \textbf{Algorithm 1: Bregman iteration}
                        \begin{itemize}
                        \item[] Initialize $p_0 = 0$ and repeat for $k = 1,2,...$
                                                \begin{flalign}
                                v_k & \in \arg\min_{v} \mathcal{F}_\xi(v) \\
                                %q_{k} & \in - \partial H(u_k) + q_{k-1} \label{eq:breg_qk}. 
                                p_{k} & \in \partial\int_{\Omega \times \Gamma} \eta(\textcolor{red}{ D v_k(x,t)}) \dint (x,t) .
                        \end{flalign}                   
                        \end{itemize}                                           
                \end{minipage}} \\
                
Due to the properties of the calibration based lifting approach Alg 1 and Alg 2 are equivalent as long as the subgradientes are chosen ``equivalent''.

We call $p_k^1$ and $p_k^2$ equivalent, if
\bfl
\langle p_k^1, u \rangle_\Omega  \quad = \quad  \langle p_k^2, G_u \rangle_{\Omega\times\Gamma}.
\efl
For the LHS it holds
\bfl
\langle p_k^1, u \rangle_\Omega  \quad = \into p_k^1(x)u(x) \dx.
\efl
For the RHS we calculate
\bfl
\langle p_k^2, G_u \rangle_\Omega  \quad &= \int_{\Omega\times\Gamma} p_k^2(x,t)G_u(x,t) \dint (x,t) \\
&= \into \int_\Gamma p_k^2(x,t)G_u(x,t) \dt \dx \\
&=  \into \int_{\R_-} p_k^2(x,t)G_u(x,t) \dt \dx \\  & \quad + \into \int_{\R_+} p_k^2(x,t)G_u(x,t) \dt \dx 
\efl
It would make sense to have $p_k^2(x,t) = 0$ for $t< 0$. In this case we are left with the second integral:
\bfl 
\langle p_k^2, G_u \rangle_\Omega  \quad &= \quad \into \int_{\R_+} p_k^2(x,t)G_u(x,t) \dt  \dx \\
&= \quad \into \int_0^{u(x)} p_k^2(x,t) \dt  \dx 
\efl
It would make sense to have $p_k^2(x,t) \equiv p_k^1(x)$. In this case we would have:
\bfl 
\langle p_k^2, G_u \rangle_\Omega  \quad 
&= \quad \into p_k^1(x) \int_0^{u(x)} 1 \dt  \dx \\
&= \quad \into p_k^1(x) u(x)  \dx \\
&= \quad \langle p_k^1(x), u(x) \rangle .
\efl

We \textbf{have seen} that $p_k^1$ and $p_k^2$ are equivalent, if
\bfl
p_k^2(x,t) = \begin{cases}
0, & t< 0 \\
p_k^1(x,t), & t < u(x).
\end{cases}
\efl 
we \textbf{don't know} whether 
\bfl
p_k^1 \in \partial J(u) \quad \Rightarrow \quad p_k^2 \in \partial J(G_u)
\efl
holds.



==> Sections/figure_bike_iso_L5n.tex <==


\begin{figure}[t]
    \begin{subfigure}{.23\linewidth}
    	\centering
    	\includegraphics[width = \linewidth]{./Images/numerical_results/bike/isotropic/none/bike_1}
    \end{subfigure}%
    \hspace{0.2cm}% Space between image A and B
    \begin{subfigure}{.23\linewidth}
    	\centering
    	\includegraphics[width = \linewidth]{./Images/numerical_results/bike/isotropic/none/bike_6}
    \end{subfigure}%
    \hspace{0.2cm}% Space between image A and B
    \begin{subfigure}{.23\linewidth}
        \centering
        \includegraphics[width = \linewidth]{./Images/numerical_results/bike/isotropic/none/bike_11}
    \end{subfigure}%
    \hspace{0.2cm}% Space between image A and B     
    \begin{subfigure}{.23\linewidth}
    	\centering
        \includegraphics[width = \linewidth]{./Images/numerical_results/bike/isotropic/none/bike_30}
    \end{subfigure}%
    \caption{\textbf{Lifted Bregman on stereo matching problem with isotropic TV.} TV-\eqref{eq:problem} with data term \eqref{eq:stereo_matching_data_term}. The problem is non-convex and non-linear in $u$. We perform the lifting with $L=4$ equidistant labels and use untransformed subgradients. Left to right: Solution at iteration $k \in \{ 1,6,11,30 \}$. For $k=1$ the solution is a vague approximation of the depth proportions. As the iteration continues more and more details are recovered. Albeit the original problem is not of the form OH-\eqref{eq:problem}, the results visually remind of an inverse scale space flow. \newline 
%
The input images are taken from the 2014 Middleburry stereo datasets \cite{data_middlebury_bike} and we use the \texttt{prost} library  \cite{sublabel_cvpr}. }
\label{fig:results2}
\end{figure}



==> Sections/lifted_breg_me.tex <==
\section{Equivalence of the Lifted Bregman Iteration}
\label{sec:lifted_bregman}

\dbdetail

An interesting question is to find  conditions under which the Bregman iteration (Alg.~1) and the more general lifted Bregman iteration (Alg.~2) are equivalent in the following sense:
If $u_k$ is a solution of the original Bregman iteration, then its lifted representation (i.e. the complete graph $\bs{1}_{u_k}$ in the fully continuous setting) is a solution of the lifted Bregman iteration. The exact definition is not trivial, as there is potential ambiguity in choosing the subgradient-based  (Bregman) term in the lifted setting.

We consider both a fully continuous and a half-discretized version of the lifted Bregman iteration, building on the theory of calibration based lifting and sublabel-accurate discretization thereof. In both cases we propose a sufficient condition on the subgradients used in the Bregman iteration. The key observation is that the Bregman iteration amounts to extending the data term by a linear term. In the half-discretized setting we prove that the condition is met in case of the anisotropic TV regularizer (see chapter 4). 

\dbnew

\subsection{Continuous Formulation}

\db{v, Gu Schreibweise einheitlich machen}
\db{Voraussetzungen: W11}

\subsubsection{Subdifferential of TV}
\label{sss:subdiff_tv}

We first review several results regarding the subdifferential of the total variation. \dbvor For simplicity, we restrict ourselves to the case $u\in W^{1,1}$ and $\Omega \subseteq \R^2$, such that $W^{1,1}(\Omega) \hookrightarrow L^2(\Omega)$ by the Sobolev embedding theorem \cite[Thm.~10.9]{book_alt}. \dbnew This allows to consider the reflexive space $L^2$ instead of the non-reflexive $W^{1,1}$. The total variation $TV: W^{1,1}(\Omega; \R) \to \Rc$,

\begin{align}
TV(u) &:= \sup_{\substack{\psi \in C_c^\infty(\Omega; \, \R^d), \\  \|\psi (x) \|_2 \leq 1}}  \into \langle u, - \text{div } \psi \rangle \dx,
\end{align}
can be viewed as a support function:
\begin{align}
&\TV(u) = \sigma_\Psi (u) \\
&\Psi := \ls - \mydiv \psi \middle| \psi \in C_c^\infty(\Omega; \, \R^d) ,  \|\psi \|_\infty \leq 1 \rs .
 \label{eq:Psi_TV}
\end{align}
Using the relation $\sigma_C \overset{*}{\longleftrightarrow} \delta_C$ \cite{book_ekeland}[Def.~I.4.1, Example I.4.3], its Fenchel conjugate is  
\begin{align}
&\TV^*(p) = \sigma^*_\Psi (p) = \delta^{**}_{\Psi} (p) = \delta_{\mycl \Psi} (p). 
\label{eq:fenchel_tv}
\end{align}
According to \cite[Prop.~I.5.1]{book_ekeland} it holds $p\in\partial\TV(u)$ iff 
\begin{align}
\TV(u) =  \langle u, p \rangle - \delta_{\mycl \Psi}(p).
\end{align}
The closure of $\Psi$ with respect to the $L^2$ norm (note that we have restricted ourselves to $L^2$) is \cite[proof of Prop.~7]{bredies2016pointwise} 
\bfl
\mycl \Psi = \ls - \mydiv \psi \, | \, \psi \in W_0^2 (\mydiv; \Omega) , \, \| \psi \|_\infty \leq 1\rs ,
\efl
where
\begin{align}
W^2 (\mydiv; \Omega) &:= \ls \psi \in L^2(\Omega, \R^d) \, | \,  \mydiv \psi \in L^2(\Omega) \rs , \\
\| \psi \|_{W^2 (\mydiv)} &:= \| \psi \|_{L^2}^2 + \| \mydiv \psi \|_{L^2}^2, \\
W_0^2 (\mydiv; \Omega) &:= \overline{C_c^\infty(\Omega; \R^d)}^{\| \cdot \|_{W^2 (\mydiv)}}.
\end{align}
\db{geändert:} Consequently, in our setting where $u\in W^{1,1}\subset L^2$, we know that $p\in L^2$ is a subgradient iff $p = -\mydiv \psi$ for some $\psi\in W_0^2(\mydiv;\Omega)$ that satisfies $\|\psi\|_\infty \leq 1$. Furthermore, it holds $TV(u)=\langle u, -\mydiv \psi\rangle_{L^2}$ \cite[Prop.~7]{bredies2016pointwise}.

%Consequently, in our setting, we know that for any $u\in W^{1,1}\subset L^2$ the subdifferential $\partial \TV(u)$ consists of all $u^\ast\in L^2$ \db{?} of the form $u^\ast = -\mydiv \psi$ for some $\psi\in W_0^2(\mydiv;\Omega)$ that satisfy $\|\psi\|_\infty \leq 1$ and $TV(u)=\langle u, -\mydiv \psi\rangle_{L^2}$ \db{?} \cite[Prop.~7]{bredies2016pointwise}.

\subsubsection{Lifted Bregman iteration}
Let us now present the lifted formulation of the Bregman iteration in a fully continuous setting. To this end we consider \eqref{eq:breg_uk} and assume that a subgradient $p_{k-1}$ is given. \dbvor Furthermore, we assume for simplicity that each subgradient $p_{k-1}$ can be represented as a $C_0(\Omega\times\R)$ function and leave the general case to future work. Using a limit argument this could also be extended to subgradients. Here we focus on the intuition...  \dbnew Since the linear Bregman term only depends on $u$, we regard it as part of the data term. Using the theory of calibration-based lifting \eqref{eq:lifted_Fxt}-\eqref{eq:constraint_set_Kt}, the energy that is minimized in %lifted equivalent  is:
\eqref{eq:breg_uk_lifted} is:
\begin{align}\label{eq:FvK}
\mathcal{F}(v) &= \sup_{\substack{\phi_x \in \mathcal{K}_x \\ \phi_t \in \mathcal{K}_t}} \int_{\Omega \times \Gamma} \left\langle \begin{pmatrix}
\phi_x \\ \phi_t
\end{pmatrix}, Dv \right\rangle , \\
\begin{split}
\label{eq:K_x}
\mathcal{K}_x &:= \{ \phi_x \in  C_0(\Omega\times\R; \R^d):  \\ &\qquad  \phi_x(x,t) \in \text{dom} \{ \eta^* \}, \quad \forall (x,t) \in \Omega\times\R \}, \end{split} \\
\begin{split} \mathcal{K}_t &:= \{ \phi_t \in  C_0(\Omega\times\R; \R ):  \\ &\qquad  - \phi_t(x,t) + tp_{k-1}(x) \leq \rho(x,t), \\ & \qquad \text{a.e. } x\in\Omega, \forall (x,t) \in \Omega\times\R \} \db{x} \label{eq:K_t}\end{split}
\end{align}
%
%
%
\jl{Kurze Bemerkung warum?}
\jl{Hier haben wir ein kleines Problem: $p_{k-1}$ ist eine $L^2$-Funktion und nicht unbedingt stetig/nur fast ueberall definiert. D.h. (40) kann nur fast ueberall gelten. Das Bloede ist aber, dass $Dv$ nicht absolutstetig bzgl. Lebesque-Mass ist, d.h. eigentlich brauchen wir $|Dv|$-fast ueberall. Oder andersrum, das Integral (38) ist (Gauss) $\int \langle \mydiv(...), v \rangle d x$. Da $p_{k-1}$ aber nur $L^2$\$nicht stetig ist, gibt es $\mydiv$ nicht. }


\input{Sections/missing_proofs.tex}

\subsubsection{Lifted TV}
\label{sss:lifted_tv}

In this section we derive the lifted formulation of the TV regularizer. Therefore, we use \eqref{eq:lifted_Fxt}-\eqref{eq:constraint_set_Kt} and set $\rho \equiv 0$:
\begin{align}
\mathcal{TV}(v) &:= \sup_{\substack{\phi_x \in \mathcal{K}_x \\ \phi_t \in \mathcal{K}_t}} \int_{\otg} \ll \begin{pmatrix} \phi_x \\ \phi_t \end{pmatrix}, Dv \rr,  \\
\begin{split} \mathcal{K}_x := \{ & \phi_x \in  C_0(\Omega\times\R; \R^d):  \\ & \phi_x(x,t) \in \text{dom} \{ \eta^* \}, \quad \forall(x,t) \in  \Omega\times\R \},  \end{split} \label{eq:Kx_TV}\\
\begin{split} \mathcal{K}_t := \{ & \phi_t \in  C_0(\Omega\times\R; \R): \\  &\phi_t(x,t) \geq 0,  \quad \forall (x,t) \in \Omega\times\R \}. \end{split} \label{eq:Kt_TV}
\end{align}
Let us assume that $u$ is smooth. We can apply \eqref{eq:Dv}-\eqref{eq:nu} and use the definition of the constraint sets \eqref{eq:Kx_TV}-\eqref{eq:Kt_TV} in order to see that $\phi_t\equiv 0$:
\begin{align}
\mathcal{TV}(v) &= \sup_{\substack{\phi_x \in \mathcal{K}_x \\ \phi_t \in \mathcal{K}_t}} \int_{\Gamma_u} \ll \begin{pmatrix} \phi_x \\ \phi_t \end{pmatrix}, \begin{pmatrix} \nabla u(x) \\ -1 \end{pmatrix} \rr \frac{\dH^d}{\sqrt{1+\|\nabla u\|^2}}   \\
\db{??} &=  \sup_{\substack{\phi_x \in C_0(\otg; \, \R^d) \\ \| \phi_x(x,t) \|_2 \leq 1}} \int_{\Gamma_u} \ll  \phi_x , \nabla u(x)  \rr \frac{\dH^d}{\sqrt{1+\|\nabla u\|^2}} \\
&=  \sup_{\substack{\phi_x \in C_0(\otg; \, \R^d) \\ \| \phi_x(x,t) \|_2 \leq 1}} \intog \ll \phi_x, (Dv)_x \rr .
\end{align}
%Applying the definition of the distributional derivative, switching the supremum with the infimum we get
%\begin{align}
%\mathcal{TV}(v) &=  \sup_{\substack{\phi_x \in C_0(\otg; \, \R^d) \\ \| \phi_x(x,t) \|_2 \leq 1}} \intog \ll - \mydivx \phi_x, v \rr \dxt \\
%&= \inf_{\substack{\phi_x \in C_0(\otg; \, \R^d) \\ \| \phi_x(x,t) \|_2 \leq 1}} \int_\Gamma \into \ll \mydivx \phi_x, v \rr \dx \dt .
%\end{align}
%\db{todo}
%\begin{align}
%\mathcal{TV}(v) &=  \int_\Gamma  \inf_{\substack{\phi \in C_0(\Omega; \, \R^d) \\ \| \phi(x) \|_2 \leq 1}} \into \ll \mydivx \phi, v \rr \dx \dt,
%\end{align}
%which shows due to the generalized coarea formula the equality
Furthermore, according to \cite[Thm.~3.2]{lifting_global_solutions}, the equality 
\bfl
\mathcal{TV}(\bs{1}_u) = \TV(u)
\label{eq:tv_equality}
\efl
holds for any $u\in W^{1,1}$. 
%, which implies
%\begin{align}
%\mathcal{TV}(G_u) &=  \sup_{\substack{\phi_x \in C_0(\otg; \, \R^d) \\ \| \phi_x(x,t) \|_2 \leq 1}} \intog \ll - \mydivx \phi_x, Gu \rr \dxt \\
%&= \inf_{\substack{\phi_x \in C_0(\otg; \, \R^d) \\ \| \phi_x(x,t) \|_2 \leq 1}} \int_\Gamma \into \ll \mydivx \phi_x, Gu \rr \dx \dt \\
% &=  \int_\Gamma  \inf_{\substack{\phi \in C_0(\Omega; \, \R^d) \\ \| \phi(x) \|_2 \leq 1}} \into \ll \mydivx \phi, Gu \rr \dx \dt = TV(u)
%\end{align}

\subsubsection{Sufficient Condition for Equivalence}
\label{sss:sufficient_continuous}

The following proposition shows that Alg.~1 and the fully continuous formulation of Alg.~2 are equivalent as long as the subgradients used in either setting fulfil a certain condition. \jl{We have to assume unique solvability of the original problem, as is the case for strictly convex functionals such as ROF.}

\db{Prop umformulieren?}
\jl{Die Notation is durcheinander, oder? Hier ist es $u,v$, oben $u$ und $\bf{u}$ (auch fuer $J$)!}

\begin{proposition} Assume that the minimization prob-\linebreak lems~\eqref{eq:breg_uk} in the original Bregman iteration have unique solutions $u_k$. Moreover, assume that the solutions $v_k$ in the lifted iteration \eqref{eq:breg_uk_lifted} are \emph{integral,} i.e., indicator functions of subgraphs $v_k = \bs{1}_u$ of some $u\in W^{1,1}$. If the chosen subgradients $p_{k-1}\in\partial \TV (u_{k-1})$ and $\bar{p}_{k-1} \in \partial \mathcal{TV} (v_{k-1})$ satisfy 
\bfl 
\bar{p}_{k-1}(\cdot,t) = p_{k-1}(\cdot), \quad \text{for a.e. } t \in \Gamma ,
\label{eq:lifted_grad_cont}
\efl
then the iterates $v_k$ of the lifted Bregman iteration are the indicator functions of the subgraphs of the iterates $u_k$ of the original Bregman iteration, i.e., $v_k = \bs{1}_{u_k}$. \jl{Do we need $v_0 = G_{u_0}$?} \\ \db{Folgt aus 1dtg der Lsg und Eigenschaften des Cal.Liftings.}
\label{prop:equivalency_cont}
\end{proposition}
\begin{proof}
From section \ref{sss:subdiff_tv}, we know that $p_{k-1}\in\mycl \Psi$.
 
\dbnew
Substituting $\tilde{\phi}_t(x,t) := \phi_t(x,t) - tp_{k-1}(x)$ into \eqref{eq:FvK}--\eqref{eq:K_t},  we arrive at the formulation 
\begin{align}
\label{eq:lifted_linear_term}
 \mathcal{F}(v) &= \sup_{\substack{\phi_x \in \mathcal{K}_x \\ \tilde{\phi_t} \in \mathcal{K}_t}} \intog  \left\langle \begin{pmatrix} \phi_x(x,t) \\ \tilde{\phi_t}(x,t) \end{pmatrix}, Dv \right\rangle +  tp_{k-1}(x) (Dv)_t ,  \\
\begin{split}
\mathcal{K}_x &:= \{ \phi_x \in  C_0(\Omega\times\R; \R^d):  \\ &\qquad  \phi_x(x,t) \in \text{dom} \{ \eta^* \}, \quad \forall (x,t) \in \Omega\times\R \}, \end{split} \\
\begin{split} \mathcal{K}_t &:= \{ \tilde{\phi_t} \in  C_0(\Omega\times\R; \R ):  \\ &\qquad  - \tilde{\phi_t}(x,t) \leq \rho(x,t), \quad \forall (x,t) \in \Omega\times\R \}. \end{split}
\end{align}

\db{Todo:}
Note that $\tilde{\phi}_t$ can be restricted to $C_0$ as well: $p_{k-1}$ is a $L^2$ function an can be uncan be uniformly approximated For any $\tilde{\phi}_t$, we can  

% Here, we have used that $p_{k-1}\in\mycl\Psi$ and the fact that $C_c^\infty$ is dense in $C_0$. \db{Noch nicht sauber , Quelle?}


Next, we want to express the second linear term in \eqref{eq:lifted_linear_term} w.r.t~ $v$, in case that $v$ is in indicator function of the subgraph of $u$. With the definition of the distributional derivative it follows
\begin{align}
&\intog \ll tp_{k-1}(x) , (Dv)_t \right\rangle \\
&= \int_\Gamma \ll - p_{k-1} , v(\cdot,t) \rr \dt .
\end{align}
%$\Gamma_u$ is a $C^1$ area \db{muss ich das zeigen?}. Using the parametrization $\gamma : \Omega\subset \R^d \to \R^{d+1}$, $\gamma(x) \mapsto \begin{pmatrix} x \\ u(x) \end{pmatrix}$
%with 
%\begin{align}
% \text{det} & \left( \left(\nabla \gamma(x)\right)^\top \nabla \gamma(x) \right) \\
%&= \text{det} \left( \begin{pmatrix} I &  \nabla u \end{pmatrix} \begin{pmatrix} I \\ (\nabla u)^\top \end{pmatrix} \right) \\
%&= \text{det} \left( I + \nabla u (\nabla u)^\top \right) \\
%&= 1 +  (\nabla u)^\top \nabla u = 1 + \| \nabla u \|^2 
%\end{align}
%we rewrite the integral as
%\begin{align}
%\int_{\Gamma_u} \frac{-tp_{k-1}(x)}{\sqrt{1+\|\nabla u(x)\|^2}} \dint \Hd^d = \into \ll -u, p_{k-1}(x) \rr \dx. 
%\end{align}
Coupling the constraint sets $\K_x$ and $\K_t$ and introducing $\bar{p}_{k-1}:\otg\to\R$, with  $\bar{p}_{k-1}(\cdot,t) := p_{k-1}(\cdot)$ for a.e. $t\in\Gamma$, the lifted Bregman iteration reads
\begin{align}
\mathcal{F}(v) &= \sup_{\phi \in \K} \intog \left\langle \phi, Dv \right\rangle - \ll \bar{p}_{k-1}, v \rr, \\
\begin{split}
\mathcal{K} &:= \{ (\phi_x, \phi_t) \in  C_0(\Omega\times\R; \R^d\times\R ):  \\ & \phi_t(x,t) + \rho(x,t) \geq \eta^*(\phi_x(x,t)), \\ & \forall (x,t) \in \Omega\times\R \} . \end{split}
\end{align}
Under the assumptions given in Prop.~\ref{prop:equivalency_cont} this concludes the proof. \qed
\end{proof}


\subsubsection{Subgradients fulfilling sufficient condition}

\db{Section in Theorem + Beweis unterteilen}

In section \ref{sss:sufficient_continuous}, Prop.~\ref{prop:equivalency_cont} we required a sufficient condition on the subgradients $p$ and $\bar{p}$. In this section, we deduce the existence of a subgradient $\bar{p}$ which fulfils the sufficient condition for $J=\TV$.

For fixed $p\in\partial \TV(u)\subseteq BV^\ast(\Omega)$ we define $\bar{p}\in BV^\ast(\Omega\times\Gamma)$ by $\langle \bar{p}, v \rangle := \int_\Gamma \ll p, v(\cdot,t) \rr dt$. If $p$ is a function, this corresponds to setting $\bar{p}$ to constant copies of $p$ along the $\Gamma$ axis, i.e., $\bar{p}(x,t):=p(x)\, \, \forall t\in\Gamma$.
Similar to the previous paragraphs, \dbvor if $u$ is a $W^{1,1}$ and therefore (in our setting) $L^2$ function, and using our general simplifying assumption that $p\in L^2(\Omega)$ \dbnew \jl{verify consistency}, we know that $\bar{p}\in L^2(\Omega\times\Gamma)$ as defined due to the boundedness of $\Gamma$.

Therefore, similar to \cite[Prop.~7]{bredies2016pointwise} and \cite[Example I.4.3, Prop.~I.5.1]{book_ekeland}, $\bar{p}$ is a subgradient of $\mathcal{TV}$ at $\bs{1}_{u}$ iff
\bfl
\mathcal{TV}(\bs{1}_{u}) = \ll \bar{p}, \bs{1}_{u} \rr - \mathcal{TV}^*(\bar{p}).
\label{eq:to_show}
\efl
%
From section \ref{sss:lifted_tv}, we recall 
\begin{align}\label{eq:psixdef}
&\mathcal{TV}(v) = \sup_{z\in\Phi_x} \intog \ll z, v \rr \dxt = \sigma_{\Phi_x} (v) \\
 &\Phi_x := \{ -\mydivx \phi_x |  \phi_x \in C_0(\otg; \, \R^d) ,   \| \phi_x(x) \|_2 \leq 1 \} 
\end{align}
and, therefore,
\begin{align}
\mathcal{TV}^*(\bar{p}) &= \delta_{\mycl \Phi_x} (\bar{p}),
\end{align}
where the closure is taken with respect to the $L^2(\Omega\times\Gamma)$ norm. 
Therefore, if we can show that $\bar{p}\in \mycl \Phi_x$ and $\mathcal{TV}(\bs{1}_{u}) = \ll \bar{p}, \bs{1}_{u} \rr$, by \eqref{eq:to_show} we know that $\bar{p}\in\partial \mathcal{TV}(\bs{1}_{u})$.

The fact that $\bar{p} \in \mycl \Phi_x$ follows directly from $p \in \mycl \Psi$ with $\Psi$ as in \eqref{eq:Psi_TV}: For every sequence $\Psi\supset\left(p_n\right) \to p$ we have a sequence $\psi_n$ of $C_c^\infty(\Omega)$ functions with $\|\psi(x)\|_2\leq 1$ and $p_n=-\mydiv \psi_n$. Thus we can set $(\phi_x)_n(x,t):=\psi_n(x)$, so that $-\mydiv_x (\phi_x)_n\in\Phi_x$ from \eqref{eq:psixdef} and $-\mydiv_x (\phi_x)_n (x,t) = -\mydiv \psi_n(x)=p_n(x)$. Thus $-\mydiv_x (\phi_x)_n(\cdot,t)\to p$ in $L^2(\Omega)$ for all $t\in\Gamma$. Due to the boundedness of $\Gamma$, this implies $-\mydiv_x (\phi_x)_n \to \bar{p}$ in $L^2(\Omega\times\Gamma)$, which shows $\bar{p}\in\mycl \Phi_x$ as desired. 

In order to show the final missing piece, i.e., $\mathcal{TV}(\bs{1}_{u}) = \ll \bar{p}, \bs{1}_{u} \rr$, note that
% \p  can define $\bar{p}_n(x,t):=p_n(x)$ for all $t\in\Gamma$. Due to the boundedness of $\Gamma$, this implies $$\bar{p}_n \to set $_{n\in\N}$ with ß
% \bfl
%         \lim_{n\to\infty} \| p_n \|_{W^2(\mydiv)} = \| p \|_{W^2(\mydiv)} 
% \efl
% we define $\left(\bar{p}_n\right)_{n\in\N}$ as $\bar{p}_n (\cdot, t) := p_n(\cdot), \, \forall t \in \Gamma$. Since $\Gamma$ is bounded and all $p_n$ are constant with respect to the second variable for all $t \in \Gamma$, it holds $\bar{p}_n \in C_0(\otg; \R^d)$ and
% \begin{align}
%         &\lim_{n\to\infty} \| \bar{p}_n \|_{W^2(\mydivx)} \\
%         &=  \lim_{n\to\infty} \into \int_\Gamma \left( \bar{p}_n(x,t) \right)^2 + \left( \mydivx \bar{p}_n(x,t) \right)^2 \dt \dx \\
%         &=  \lim_{n\to\infty} \into | \Gamma | \left( \left( p_n(x) \right)^2 + \left( \mydiv p_n(x) \right)^2 \right)  \dx \\
%         &=  \into | \Gamma | \left( \left( p(x) \right)^2 + \left( \mydiv p(x) \right)^2 \right) \dx \\
%         &=  \intog \left( \bar{p}(x,t) \right)^2 + \left( \mydivx \bar{p}(x,t) \right)^2 \dt \dx \\
%         &= \| \bar{p} \|_{W^2(\mydivx)}.
% \end{align}
%With \eqref{eq:tv_equality} and the coarea formula the rest of \eqref{eq:to_show} follows:
\begin{align}
\mathcal{TV}(\bs{1}_{u}) &\overset{\eqref{eq:tv_equality}}{=} \TV(u) = \ll p, u \rr\\
 & \overset{(*)}= \int_\Omega p(x) \int_\Gamma \bs{1}_{u}(x,t) \dt \dx\\
 & = \langle \bar{p}, \bs{1}_{u}\rangle.
\end{align}
The crucial step is $(*)$, where we again used a coarea-type formula for linear terms.

Therefore, by defining $\bar{p}$ based on $p$ as above, we have recovered a subgradient of the lifted regularizer $\mathcal{TV}$ of the form required by Prop.~\ref{prop:equivalency_cont}.



%
%\subsubsection{Properties of Calibration based lifting}
%\db{Unnötig, aber die letzte Gleichung ist spannend.}
%
%Let us recall the lifted Bregman iteration:
%\begin{align}
%\mathcal{F}(v) &= \sup_{\substack{\phi_x \in \mathcal{K}_x \\ \phi_t \in \mathcal{K}_t}} \int_{\Omega \times \Gamma} \left\langle \begin{pmatrix}
%\phi_x \\ \phi_t
%\end{pmatrix}, Dv \right\rangle , \\
%\begin{split}
%\mathcal{K}_x &:= \{ \phi_x \in  C_0(\Omega\times\R; \R^d):  \\ &\qquad  \phi_x(x,t) \in \text{dom} \{ \eta^* \}, \quad \forall (x,t) \in \Omega\times\R \}, \end{split} \\
%\begin{split} \mathcal{K}_t &:= \{ \phi_t \in  C_0(\Omega\times\R; \R ):  \\ &\qquad  - \phi_t(x,t) + tp_{k-1}(x) \leq \rho(x,t), \\ & \qquad \forall (x,t) \in \Omega\times\R \} \end{split}.
%\end{align}
%The $\phi_x$, $\phi_t$ maximizing the function are called \emph{calibrations} and are in fact divergence free, i.e. 
%\begin{align}
%\mydiv \begin{pmatrix}
%\phi_x \\ \phi_t
%\end{pmatrix} = \mydiv \phi_x + \frac{\text{d}}{\dt} \phi_t = 0.
%\end{align}
%Using the substitution $\tilde{\phi}_t(x,t) := \phi_t(x,t) - t p_{k-1}(x)$
%\begin{align}
%\mydiv \begin{pmatrix}
%\phi_x \\ \tilde{\phi}_t
%\end{pmatrix}  = - p_{k-1}(x) .
%\end{align}
%Due to \eqref{eq:K_x} it holds $p_k := \phi_x \in \text{dom} \ls \eta^* \rs = \mycl \Psi .$, \db{maybe even $\delta TV?$} 
%\begin{align}
%p_k(x) = - p_{k-1}(x) - \frac{\text{d}}{\dt}\tilde{\phi}_t .
%\end{align}



%\subsubsection{Subgradients fulfilling sufficient condition}
%
%\db{Großes TODO}
%
%We have just seen why it is essential to find a connection between $\partial J(u)$ and $\partial J(G_u)$, where $G_u$ is the complete graph of $u$. In this paper, we consider the total variation regularizer, i.e.
%\begin{align}
%%TV(u) &= \sup_{\substack{\psi\in C_c^\infty(\Omega; \, \R^d)\\ \|\psi (x,t) \|_2 \leq 1}} \left\{ - \into \langle u, \text{div} \psi \rangle \dx \right\} \\
%TV(G_u) &= \sup_{\substack{\psi\in C_c^\infty(\Omega\times\Gamma; \, \R^d\times\R)\\\|\psi (x,t) \|_2 \leq 1}} A(G_u, \psi) \\
%A(G_u, \psi) &:=  - \intog \langle G_u, \text{div} \psi \rangle \dxt 
%\end{align}
%%
%We apply the divergence theorem and note that $\psi$ has compact support. Furthermore we can use \eqref{eq:Dv} and the notation $\psi = (\psi_x, \psi_t)^\top$, as well as the parametrization~$\gamma$ introduced in the last section.
%\begin{align}
%\label{eq:TVGu2}
%& A(G_u, \psi) =  \intog \langle \psi,  D G_u \rangle \\
%&= \int_{\Gamma_u} \ll \begin{pmatrix} \psi_x \\ \psi_t \end{pmatrix} (x,t), \begin{pmatrix} \nabla u(x) \\ -1 \end{pmatrix} \rr \frac{\dH^d(x,t)}{\sqrt{1+\|\nabla u(x)\|^2}} \\
%&= \into \ll \begin{pmatrix} \psi_x \\ \psi_t \end{pmatrix} (x,u(x)), \begin{pmatrix} \nabla u(x) \\ -1 \end{pmatrix} \rr \dx
%\end{align}
%On the other hand we have
%\begin{align}
%TV(u) &= \sup_{\substack{\psi\in C_c^\infty(\Omega; \, \R^d)\\ \|\psi (x) \|_2 \leq 1}}\left\{ - \into \ll u(x), \mydiv \psi(x) \rr \dx \right\} \\
%&= \sup_{\substack{\psi\in C_c^\infty(\Omega; \, \R^d)\\ \|\psi (x) \|_2 \leq 1}}\left\{  \into \ll \psi, \nabla u \rr  \right\} \dx
%\end{align}
%\db{TODO:}
%Basically we would need $\mydiv \psi (x) = p_{k-1}(x) \Rightarrow \mydiv \begin{pmatrix} \psi_x \\ \psi_t \end{pmatrix} (x,t) = -p_{k-1}(x)$
%
%\db{neuer Ansatz}
%
%Assuming we have a fixed $\psi$, such that 
%\begin{align}
%TV(u) = \into \ll u, -\mydiv \psi \rr \dx,
%\end{align}
%we define $p_{k-1} := -\mydiv \psi$. It holds $p_{k-1} \in \partial \TV (u)$. The proof, that $\bar{p}_{k-1} \in \partial \TV(G_u)$ holds, is twofold. We begin by showing, that $TV(G_u) = \intog \ll G_u, -\bar{p}_{k-1} \rr \dxt$:
%\begin{align}
%TV(G_u) &= \sup_{\psi \in \Psi} \intog \ll  G_u, -\mydiv \psi \rr \dxt \\
%&= \sup_{\psi \in \Psi} \intog \ll  G_u, -\mydiv \psi \rr \dxt
%\end{align}
%where
%\bfl
%\Psi &:= \ls \psi\in  C_c^\infty(\otg; \, \R^d\times\R), \, \|\psi (x,t) \|_2 \leq 1 \rs
%\efl
%\begin{enumerate}
%\item $TV(G_u) = \intog \ll G_u, -\bar{p}_{k-1} \rr \dxt$ ,
%\item $\bar{p}_{k-1} \in W_0^2(\mydiv; \otg)$.
%\end{enumerate}

\dbold

\subsection{Half-Discretized Formulation}
 
\db{Einleitung checken und anpassen}

The following considerations are formal due to the mostly pointwise arguments; we leave a rigorous investigation in the function space to future work. However, they can equally be understood in the spatially discrete setting with finite $\Omega$, where arguments are more straightforward. For readability, we consider a fixed $x \in \Omega $ and omit $x$ in the arguments.

\begin{proposition}
Assume $\rho_1,\rho_2,h: \Gamma \mapsto \Rc$ with
\begin{align}
\rho_2(u) := \rho_1 (u) - h(u), \quad h(u) := pu, \quad p\in\R,
\end{align}
where $\rho_1$ and $\rho_2$ should be understood as two different  data terms in~\eqref{eq:problem}. Define
\begin{equation}
\tilde{\bs{\gamma}} := \begin{pmatrix} \gamma_2 - \gamma_1, & \hdots, & \gamma_{L} - \gamma_l \end{pmatrix}^{\top}\label{eq:bs_gamma}
\end{equation}
Then, for the lifted representations $\bs{\rho}_1,\bs{\rho}_2,\bs{h} : \R^l \mapsto \Rc$ in \eqref{eq:def_data_integrand}, it holds %the following equality holds for the Fenchel biconjugates:
\begin{equation}
\bs{\rho}_2^{**}(\bs{u})  =  \bs{\rho}_1^{**}(\bs{u}) - \bs{h}^{**}(\bs{u})   =   \bs{\rho}_1^{**}(\bs{u}) - \langle p \tilde{\bs{\gamma}}, \bs{u} \rangle  .
\end{equation}
%i.e.,~the sum of two separately relaxed data terms is point-wise equal to the relaxation of their sum, whenever one of the data terms is linear in $u$.
\label{prop:lifted_sum}
\end{proposition}
\dbdetail
%
\begin{proof}
The proof is quite technical. We deduce the biconjugate of $\bs{\rho}_2$ step-by-step and show that the final expression implies the anticipated equality. According to \eqref{eq:def_data_integrand} the lifted representation of $\rho_2$ is
\begin{align}
\bs{\rho}_2(\textbf{u}) &= \inf_{\substack{i\in\{1,...,l\}, \\\alpha \in [0,1]}}  \left \{ \rho_2(\gamma_i^{\alpha}) + \delta_{\textbf{1}_i^{\alpha}}(\textbf{u}) \right \}.
\label{eq:def_data_integrand_sum}
\end{align}
We use the definition of the Fenchel conjugate and note that the supremum is attained for some  $\textbf{u}\in\boldsymbol{\Gamma}$:
\begin{align}
\bs{\rho}_2^*(\textbf{v}) &= \sup_{\textbf{u} \in \R^l} \left \{ \langle \textbf{u}, \textbf{v} \rangle - \bs{\rho}_2(\textbf{u}) \right \} \\
&= \sup_{\substack{j\in\{1,...,l\}, \\ \beta \in [0,1]}} \left \{ \langle \textbf{u}, \textbf{v} \rangle - \bs{\rho}_2(\textbf{u}) \right \}.
\end{align}
The definition of $\bs{\rho}_2$ and $\rho_2$ lead to:
\begin{align}
\bs{\rho}_2^*(\textbf{v}) 
&= \sup_{\substack{j\in\{1,...,l\}, \\ \beta \in [0,1]}} \left \{ \langle \textbf{1}_j^{\beta}, \textbf{v} \rangle -  \rho_1\left(\gamma_j^{\beta}\right) + p \gamma_j^{\beta} \right \} .
\end{align}
Using $\tilde{\bs{\gamma}}$ as in \eqref{eq:bs_gamma} we can furthermore express $p\gamma_j^{\beta} $ in terms of $\textbf{1}_j^{\beta}$:
\begin{align}
\bs{\rho}_2^*(\textbf{v}) &= \sup_{\substack{j\in\{1,...,l\},\\ \beta \in [0,1]}} \left \{ \langle \textbf{1}_j^{\beta}, \textbf{v} \rangle - \rho_1\left(\gamma_j^{\beta}\right) + \langle p \tilde{\bs{\gamma}} , \textbf{1}_j^{\beta} \rangle  \right \} \\
&= \sup_{\substack{j\in\{1,...,l\}, \\ \beta \in [0,1]}} \left \{ \langle \textbf{1}_j^{\beta}, \textbf{v} + p \tilde{\bs{\gamma}} \rangle - \rho_1\left(\gamma_j^{\beta}\right) \right \}.
\end{align}
Next we compute the biconjugate of $\bs{\rho}$:  
\begin{align}
\bs{\rho}_2^{**}(\textbf{w}) &= \sup_{\textbf{v} \in \R^l} \left \{\langle \textbf{v}, \textbf{w} \rangle - \bs{\rho}_2^*(\textbf{v}) \right \} .
\end{align}
By substituting $\textbf{z} := \textbf{v} + p \tilde{\bs{\gamma}} $ we get
\begin{align}
\bs{\rho}_2^{**}(\textbf{w}) =  &
\sup_{\textbf{z} \in \R^l} \Bigg \{ \langle \textbf{z} -p \tilde{\bs{\gamma}}, \textbf{w} \rangle  \\ &   -   \sup_{\substack{j\in\{1,...,l\}, \\ \beta \in [0,1]}} \left \{ \langle \textbf{1}_j^{\beta}, \textbf{z}  \rangle - \rho_1\left(\gamma_j^{\beta}\right) \right \} \Bigg \} \\
= & - \langle \textbf{w}, p \tilde{\bs{\gamma}} \rangle + \sup_{\textbf{z} \in \R^l} \Bigg \{ \langle \textbf{z} , \textbf{w} \rangle  \\ &  - \sup_{\substack{j\in\{1,...,l\}, \\ \beta \in [0,1]}} \left \{ \langle \textbf{1}_j^{\beta}, \textbf{z}  \rangle - \rho_1\left(\gamma_j^{\beta}\right) \right \}  \Bigg  \}  \\
= & \bs{\rho}_1^{**}(\textbf{w}) - \langle \textbf{w}, p \tilde{\bs{\gamma}} \rangle .
\end{align}
In reference to \cite[Prop.~2]{sublabel_cvpr} we see, that the expression $ \langle \textbf{w}, p \tilde{\bs{\gamma}} \rangle $ is in fact $\textbf{h}^{**}(\textbf{w})$. This concludes the proof of Thm.~\ref{prop:lifted_sum}. \qed
\end{proof}
%
\dbold

The following proposition shows that Alg.~1 and Alg.~2 are equivalent as long as we base the iteration on subgradients $p_{k-1}$ and $\bs{p}_{k-1}$ in the subdifferential of $J(u_{k-1})$ and $\bs{J}(\bs{u}_{k-1})$ that are linked in a particular way.

\begin{proposition} Assume that the minimization problems \eqref{eq:breg_uk} in the original Bregman iteration have unique solutions. Moreover, assume that in the lifted iteration, the solutions $\bs{u}_k$ of \eqref{eq:breg_uk_lifted} in each step satisfy $\bs{u}(x)\in\bs{\Gamma}$, i.e., are sublabel-integral. If at every point $x$ the chosen subgradients $p_{k-1}\in\partial J(u_{k-1})$ and $\bs{p}_{k-1} \in\partial \bs{J}(\bs{u}_{k-1})$ satisfy 
%For the ROF-\eqref{eq:problem} problem, the iterates $u_k$ and $\bs{u}_k$ determined by \eqref{eq:breg_uk} and \eqref{eq:breg_uk_lifted} are equivalent as long as 
\bfl 
\bs{p}_{k-1}(x) \quad = %\quad p_{k-1} \begin{pmatrix} \gamma_2 - \gamma_1, & \hdots, & \gamma_{l+1} - \gamma_{l} \end{pmatrix}^\top
\quad p_{k-1}(x) \tilde{\bs{\gamma}} 
\label{eq:lifted_grad}
\efl
with $\tilde{\bs{\gamma}}$ as in \eqref{eq:bs_gamma}, then the lifted iterates $\bs{u}_k$ correspond to the iterates $u_k$ of the classical Bregman iteration \eqref{eq:breg_uk} according to \eqref{eq:projection}.
%holds for the subgradients . Here, $u_{k-1}$ and $\bs{u}_{k-1}$ denote the minimizers of the previous iteration.
\label{prop:equivalency}
\end{proposition}

\begin{proof}[Proof of Proposition \ref{prop:equivalency}]
We define the \emph{extended data term}
\begin{equation}
\tilde{H}(u) := \into \rho(x,u(x)) - p(x) u(x) \dx,
\end{equation}
which incorporates the linear term of the Bregman iteration.
Using Prop.~\ref{prop:lifted_sum}, we reach the following lifted representation:
\begin{align}
\tilde{\bs{H}}(\bs{u}) &= \into \bs{\rho}^{**}(x,\bs{u}(x)) - \langle p(x)\tilde{\bs{\gamma}}, \bs{u}(x) \rangle \dx .
\end{align}
Hence the lifted version of \eqref{eq:breg_uk} is
\begin{equation}
\arg\min_{\bs{u}\in\bs{U}} \left \{ \bs{H}(\bs{u}) +\bs{J}(\bs{u}) - \langle p_{k-1} \tilde{\bs{\gamma}}, \bs{u} \rangle  \right \}.
\end{equation}
Comparing this to  \eqref{eq:breg_uk_lifted} shows that the minimization problem in the lifted iteration is the lifted version of \eqref{eq:breg_uk} if the subgradients  $p_{k-1}\in\partial J(u_{k-1})$ and $\bs{p}_{k-1} \in\partial \bs{J}(\bs{u}_{k-1})$ satisfy $ \bs{p}_{k-1} = p_{k-1} \tilde{\bs{\gamma}}$.
 In this case, since we have assumed that the solution of the lifted problem \eqref{eq:breg_uk_lifted} is sublabel-integral, it can be associated via \eqref{eq:projection} with the solution of the original problem \eqref{eq:breg_uk}, which is unique by assumption.\qed
 
%  as in the assumptions.holds for the subgradients $.\jl{Mir ist noch nicht klar wie die spezielle Form von $\bs{p}_{k-1}$ in den Beweis eingeht}\

%In other words: Under the above mentioned assumption on the subgradients, applying the Bregman iteration on the lifted problem is equivalent to lifting the Bregman iteration \eqref{eq:breg_uk}. Assuming that the discretized lifted problem gives a solution of the original problem \jl{sollte in die Voraussetzung} this concludes the proof.

 %\db{Reicht der Satz, oder lieber etwas ausführlicher? Siehe auskommentiert.} \qed
\end{proof}
%In \cite{sublabel_discretization} it has been shown that the sublabel-accurate relaxation is in fact a special discretization of the lifting approach. % introduced in \cite{lifting_global_solutions}.The thresholded  solution of the latter is a global optimal solution of the original problem  \cite{lifting_global_solutions}. Ignoring errors introduced by the discretization, we can say, that the original and lifted Bregman iteration are equivalent, as long as the subgradients meet the assumption. \jl{Liest sich noch etwas wackelig. Ich denke das sollten wir praezisieren, in einer Annahme, z.B. dass im konvexen Fall das geliftete diskretisierte(!) Problem eine Loesung des ungelifteten Problems liefert.}
Thus, under the condition of the proposition, the lifted and unlifted Bregman iterations are equivalent.







%\db{old section deleted - see comments}
%
%\subsubsection{Old}
%
%\db{Muss noch umgeschrieben werden! Subdifferntial blabliblub}
%
%
%In order for \eqref{eq:breg_uk} and \eqref{eq:breg_uk_tilde} to be equivalent  for $k=2$ there must exist a subgradient  $q_1 \in - \partial H(u_1)$ such that
%\begin{equation}
%\bs{q}_{1} := q_{1} \begin{pmatrix}\gamma_2 - \gamma_1 \\ \vdots \\ \gamma_{l+1}- \gamma_l \end{pmatrix} \in - \partial \bs{H}(\bs{u}_1)
%\end{equation}
%We proceed with the following assumption: \jl{Hatten wir dazu nicht einen Satz (Integralform)?}
%\begin{align}
%\partial H(u_{1}) & = \partial \into \rho(x,u_1(x)) \dx \overset{!}{\supset}  \into \partial \rho(x,u_1(x)) \dx, \\
%\partial \bs{H}(\bs{u}_{1}) & = \partial \into \bs{\rho}^{**}(x,\bs{u}_1(x)) \dx \overset{!}{\supset}  \into \partial \bs{\rho}^{**}(x,\bs{u}_1(x)) \dx .
%\end{align}
%Please note, that the inclusion is in fact only known for finite sums and not for integrals \cite[Cor.~10.9]{book_rock_variational}. However, since the spatial domain needs to be discretized before the Bregman iteration anyways, we stick with this somewhat improper notation. With theorem \ref{thm:lifted_subgradient} this implies
%\begin{flalign}
%q_1 :=& \into z(x) \dx \in \partial H(u_1)  \\
%\Leftrightarrow q_1 \begin{pmatrix}\gamma_2 - \gamma_1 \\ \vdots \\ \gamma_{l+1}- \gamma_l \end{pmatrix} =& \into z(x) \begin{pmatrix}\gamma_2 - \gamma_1 \\ \vdots \\ \gamma_{l+1}- \gamma_l \end{pmatrix} \dx \in \partial \bs{H}(\bs{u}_1)
%\end{flalign}
%and thus the equivalency of \eqref{eq:breg_uk} and \eqref{eq:breg_uk_tilde} under the above mentioned assumptions. \jl{Das ist das Hauptergebnis und sollte deshalb besser sichbar sein, am besten ein eigener Satz. Eventuell sogar schon in die Introduction einbringen.} We leave a more thorough analysis of the lifted Bregman iteration to future work. 
%


==> Sections/missing_proofs.tex <==
\vspace{1cm}

\textbf{MISSING PROOF}

\noindent Subgradients $p_{k-1}$ lie in $\mycl \Psi$, i.e. $ \exists \psi\in \overline{C_c^\infty (\Omega; \R^d)}^{\| \cdot \|_{W^2(\mydiv)}}$, such that $p_{k-1} = - \mydiv \psi$. We can find a sequence $(\psi^n)_{n\in\N} \overset{\| \cdot \|_{W^2(\mydiv)}}{\longrightarrow} \psi$, with $\psi^n \in C_c^\infty$. Define $p_{k-1}^n := -\mydiv \psi^n$. It holds
\bfl
p_{k-1}^n = -\mydiv \psi^n \overset{\|\cdot\|_{L^2}}{\longrightarrow}  -\mydiv \psi = p_{k-1}.
\efl
Define 
\bfl
F^n_{\text{Breg}}(u) := F(u) - \ll p_{k-1}^n, u \rr.
\efl
IF WE COULD SHOW
\begin{align}
\lim_{n\to\infty} F^n_{\text{Breg}}(u) &= \lim_{n\to\infty} F(u) - \ll p_{k-1}^n, u \rr \\ 
& \overset{???}{=} F(u) - \ll \lim_{n\to\infty} p_{k-1}^n, u \rr \\
& = F(u) - \ll p_{k-1}, u \rr = F_{\text{Breg}}(u)
\end{align}
THEN IT WOULD FOLLOW
\begin{align}
\F^n_{\text{Breg}} &:= \sup{\phi_x, \phi_t} \intog \ll \phi, Dv \rr, \\
\K_x &= \ls ... \rs \\
\K_t &= \ls ...  -\phi_t(x,t) + tp_{k-1}^n(x) \leq \rho(x,t) ... \rs
\end{align}
and with the substitution $\tilde{\phi_t}(x,t) = \phi_t(x,t) - t p_{k-1}^n(x)$
\begin{align}
\F^n_{\text{Breg}} &:= \sup_{\phi_x, \tilde{\phi_t}} \intog \ll \phi, Dv \rr - \ll p_{k-1}^n, v \rr, \\
\K_x &= \ls ... \rs \\
\K_t &= \ls ...  -\tilde{\phi_t}(x,t) \leq \rho(x,t) ... \rs
\end{align}
and 
\begin{align*}
\lim_{n\to\infty} \F^n_{\text{Breg}}(u) &= \lim_{n\to\infty} \intog \ll \phi, Dv \rr F(u) - \ll p_{k-1}^n, v \rr \\ 
& \overset{???}{=}  \intog \ll \phi, Dv \rr F(u) - \ll \lim_{n\to\infty} p_{k-1}^n, v \rr \\
& = \intog \ll \phi, Dv \rr F(u) - \ll p_{k-1}, v \rr \\
& = \F_{\text{Breg}}(u)
\end{align*}
